Deep Integrated Explanations

This paper presents Deep Integrated Explanations (DIX) - a universal method for explaining vision models. DIX generates explanation maps by integrating information from the intermediate representations of the model, coupled with their corresponding gradients. Through an extensive array of both objective and subjective evaluations spanning diverse tasks, datasets, and model configurations, we showcase the efficacy of DIX in generating faithful and accurate explanation maps, while surpassing current state-of-the-art methods.

==> latex/tables/cikm2_cnn_segmentation2222.tex <==
\begin{table}

    \caption{Segmentation tests on three datasets (CNN models). For all metrics, higher is better. See Sec.~\ref{subsec:res_seg} for details.}
  \label{tab:cnns_segmentation_table}
   \begin{center}

   \scalebox{1}{
    \begin{tabular}{@{}lc@{}lc@{}lc@{}lc@{}lc@{}lc@{}lc@{}}
    \toprule
      & & & \multicolumn{1}{l}{GC} & \multicolumn{1}{l}{GC++} & \multicolumn{1}{l}{LIFT} & \multicolumn{1}{l}{AC} & \multicolumn{1}{l}{DIX2} & \multicolumn{1}{l}{DIX3}\\
    \midrule
    \multirow{12}{*}{\makecell{IN-SEG}}
    & \multirow{4}{*}{CN}

    & \multicolumn{1}{l}{PA} & \multicolumn{1}{l}{77.01} & \multicolumn{1}{l}{77.54} & \multicolumn{1}{l}{63.77} & \multicolumn{1}{l}{77.04} & \multicolumn{1}{l}{\underline{78.32}} & \multicolumn{1}{l}{\textbf{78.93}}\\

    & & \multicolumn{1}{l}{mAP} & \multicolumn{1}{l}{81.01} & \multicolumn{1}{l}{85.63} & \multicolumn{1}{l}{69.40} & \multicolumn{1}{l}{86.93} & \multicolumn{1}{l}{\underline{87.13}} & \multicolumn{1}{l}{\textbf{87.34}}\\

    & & \multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{56.58} & \multicolumn{1}{l}{58.35} & \multicolumn{1}{l}{53.81} & \multicolumn{1}{l}{58.42} & \multicolumn{1}{l}{\underline{58.64}} & \multicolumn{1}{l}{\textbf{58.79}}\\
    
    & & \multicolumn{1}{l}{mF1} & \multicolumn{1}{l}{36.88} & \multicolumn{1}{l}{38.26} & \multicolumn{1}{l}{35.91} & \multicolumn{1}{l}{41.29} & \multicolumn{1}{l}{\underline{42.51}} & \multicolumn{1}{l}{\textbf{42.95}}\\
    
    & \multirow{4}{*}{RN}

    & \multicolumn{1}{l}{PA} & \multicolumn{1}{l}{71.93} & \multicolumn{1}{l}{71.96} & \multicolumn{1}{l}{71.68} & \multicolumn{1}{l}{70.36} & \multicolumn{1}{l}{\underline{72.43}} & \multicolumn{1}{l}{\textbf{73.17}}\\

    & & \multicolumn{1}{l}{mAP} & \multicolumn{1}{l}{84.21} & \multicolumn{1}{l}{84.23} & \multicolumn{1}{l}{83.79} & \multicolumn{1}{l}{81.14} & \multicolumn{1}{l}{\underline{84.58}} & \multicolumn{1}{l}{\textbf{85.37}}\\

    & & \multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{53.06} & \multicolumn{1}{l}{53.29} & \multicolumn{1}{l}{52.17} & \multicolumn{1}{l}{52.91} & \multicolumn{1}{l}{\underline{53.93}} & \multicolumn{1}{l}{\textbf{54.16}}\\
    
    & & \multicolumn{1}{l}{mF1} & \multicolumn{1}{l}{42.51} & \multicolumn{1}{l}{42.68} & \multicolumn{1}{l}{41.95} & \multicolumn{1}{l}{42.08} & \multicolumn{1}{l}{\underline{42.75}} & \multicolumn{1}{l}{\textbf{43.18}}\\
    
    
    & \multirow{4}{*}{DN}

    & \multicolumn{1}{l}{PA} & \multicolumn{1}{l}{73.00} & \multicolumn{1}{l}{73.21} & \multicolumn{1}{l}{72.87} & \multicolumn{1}{l}{72.44} & \multicolumn{1}{l}{\underline{73.58}} & \multicolumn{1}{l}{\textbf{73.90}}\\

    & & \multicolumn{1}{l}{mAP} & \multicolumn{1}{l}{85.04} & \multicolumn{1}{l}{85.53} & \multicolumn{1}{l}{84.82} & \multicolumn{1}{l}{84.62} & \multicolumn{1}{l}{\underline{85.57}} & \multicolumn{1}{l}{\textbf{85.98}}\\

    & & \multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{54.18} & \multicolumn{1}{l}{54.57} & \multicolumn{1}{l}{54.11} & \multicolumn{1}{l}{54.89} & \multicolumn{1}{l}{\underline{55.42}} & \multicolumn{1}{l}{\textbf{56.03}}\\
    
    & & \multicolumn{1}{l}{mF1} & \multicolumn{1}{l}{41.74} & \multicolumn{1}{l}{42.58} & \multicolumn{1}{l}{41.61} & \multicolumn{1}{l}{43.51} & \multicolumn{1}{l}{\underline{43.71}} & \multicolumn{1}{l}{\textbf{43.79}}\\
    
    \midrule
    
    \multirow{12}{*}{COCO}

    & \multirow{4}{*}{CN}
    & \multicolumn{1}{l}{PA} & \multicolumn{1}{l}{68.75} & \multicolumn{1}{l}{66.49} & \multicolumn{1}{l}{60.37} & \multicolumn{1}{l}{64.10} & \multicolumn{1}{l}{\underline{68.87}} & \multicolumn{1}{l}{\textbf{69.38}}\\

    & & \multicolumn{1}{l}{mAP} & \multicolumn{1}{l}{75.02} & \multicolumn{1}{l}{75.21} & \multicolumn{1}{l}{67.98} & \multicolumn{1}{l}{76.09} & \multicolumn{1}{l}{\underline{76.94}} & \multicolumn{1}{l}{\textbf{77.43}}\\

    & & \multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{43.46} & \multicolumn{1}{l}{44.01} & \multicolumn{1}{l}{37.08} & \multicolumn{1}{l}{44.27} & \multicolumn{1}{l}{\underline{44.89}} & \multicolumn{1}{l}{\textbf{45.06}}\\
    
    & & \multicolumn{1}{l}{mF1} & \multicolumn{1}{l}{28.96} & \multicolumn{1}{l}{29.85} & \multicolumn{1}{l}{26.92} & \multicolumn{1}{l}{30.81} & \multicolumn{1}{l}{\underline{31.28}} & \multicolumn{1}{l}{\textbf{31.99}}\\
    
    & \multirow{4}{*}{RN}

    & \multicolumn{1}{l}{PA} & \multicolumn{1}{l}{64.17} & \multicolumn{1}{l}{64.39} & \multicolumn{1}{l}{64.02} & \multicolumn{1}{l}{63.90} & \multicolumn{1}{l}{\underline{64.75}} & \multicolumn{1}{l}{\textbf{64.94}}\\

    & & \multicolumn{1}{l}{mAP} & \multicolumn{1}{l}{74.19} & \multicolumn{1}{l}{74.27} & \multicolumn{1}{l}{73.78} & \multicolumn{1}{l}{72.80} & \multicolumn{1}{l}{\underline{74.38}} & \multicolumn{1}{l}{\textbf{74.91}}\\

    & & \multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{42.37} & \multicolumn{1}{l}{43.25} & \multicolumn{1}{l}{42.59} & \multicolumn{1}{l}{42.88} & \multicolumn{1}{l}{\underline{43.54}} & \multicolumn{1}{l}{\textbf{43.87}}\\
    
    & & \multicolumn{1}{l}{mF1} & \multicolumn{1}{l}{31.64} & \multicolumn{1}{l}{32.82} & \multicolumn{1}{l}{31.77} & \multicolumn{1}{l}{32.41} & \multicolumn{1}{l}{\underline{33.39}} & \multicolumn{1}{l}{\textbf{33.71}}\\
    
    
    & \multirow{4}{*}{DN}

    & \multicolumn{1}{l}{PA} & \multicolumn{1}{l}{63.50} & \multicolumn{1}{l}{64.06} & \multicolumn{1}{l}{63.25} & \multicolumn{1}{l}{64.51} & \multicolumn{1}{l}{\underline{64.98}} & \multicolumn{1}{l}{\textbf{65.37}}\\

    & & \multicolumn{1}{l}{mAP} & \multicolumn{1}{l}{72.61} & \multicolumn{1}{l}{73.07} & \multicolumn{1}{l}{72.15} & \multicolumn{1}{l}{73.85} & \multicolumn{1}{l}{\underline{74.02}} & \multicolumn{1}{l}{\textbf{74.67}}\\

    & & \multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{43.02} & \multicolumn{1}{l}{43.75} & \multicolumn{1}{l}{42.85} & \multicolumn{1}{l}{44.16} & \multicolumn{1}{l}{\underline{44.75}} & \multicolumn{1}{l}{\textbf{44.82}}\\
    
    & & \multicolumn{1}{l}{mF1} & \multicolumn{1}{l}{31.04} & \multicolumn{1}{l}{32.31} & \multicolumn{1}{l}{30.83} & \multicolumn{1}{l}{33.93} & \multicolumn{1}{l}{\underline{34.14}} & \multicolumn{1}{l}{\textbf{34.59}}\\
    
     \midrule
    
    \multirow{12}{*}{\makecell{VOC}}
    & \multirow{4}{*}{CN}

    & \multicolumn{1}{l}{PA} & \multicolumn{1}{l}{72.54} & \multicolumn{1}{l}{72.09} & \multicolumn{1}{l}{63.32} & \multicolumn{1}{l}{69.83} & \multicolumn{1}{l}{\underline{72.68}} & \multicolumn{1}{l}{\textbf{72.81}}\\

    & & \multicolumn{1}{l}{mAP} & \multicolumn{1}{l}{77.27} & \multicolumn{1}{l}{79.47} & \multicolumn{1}{l}{68.83} & \multicolumn{1}{l}{80.45} & \multicolumn{1}{l}{\underline{81.35}} & \multicolumn{1}{l}{\textbf{81.79}}\\

    & & \multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{50.28} & \multicolumn{1}{l}{50.63} & \multicolumn{1}{l}{48.86} & \multicolumn{1}{l}{49.76} & \multicolumn{1}{l}{\underline{51.12}} & \multicolumn{1}{l}{\textbf{51.29}}\\
    
    & & \multicolumn{1}{l}{mF1} & \multicolumn{1}{l}{35.24} & \multicolumn{1}{l}{35.67} & \multicolumn{1}{l}{33.26} & \multicolumn{1}{l}{34.51} & \multicolumn{1}{l}{\underline{35.92}} & \multicolumn{1}{l}{\textbf{36.57}}\\
    
    & \multirow{4}{*}{RN}

    & \multicolumn{1}{l}{PA} & \multicolumn{1}{l}{68.74} & \multicolumn{1}{l}{69.01} & \multicolumn{1}{l}{68.61} & \multicolumn{1}{l}{68.00} & \multicolumn{1}{l}{\underline{69.38}} & \multicolumn{1}{l}{\textbf{69.74}}\\

    & & \multicolumn{1}{l}{mAP} & \multicolumn{1}{l}{79.68} & \multicolumn{1}{l}{79.96} & \multicolumn{1}{l}{79.41} & \multicolumn{1}{l}{78.02} & \multicolumn{1}{l}{\underline{81.02}} & \multicolumn{1}{l}{\textbf{81.49}}\\

    & & \multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{49.44} & \multicolumn{1}{l}{49.91} & \multicolumn{1}{l}{49.15} & \multicolumn{1}{l}{49.32} & \multicolumn{1}{l}{\underline{50.43}} & \multicolumn{1}{l}{\textbf{51.58}}\\
    
    & & \multicolumn{1}{l}{mF1} & \multicolumn{1}{l}{33.08} & \multicolumn{1}{l}{33.56} & \multicolumn{1}{l}{32.69} & \multicolumn{1}{l}{32.74} & \multicolumn{1}{l}{\underline{34.28}} & \multicolumn{1}{l}{\textbf{34.68}}\\
    
    
    & \multirow{4}{*}{DN}

    & \multicolumn{1}{l}{PA} & \multicolumn{1}{l}{68.43} & \multicolumn{1}{l}{68.78} & \multicolumn{1}{l}{68.24} & \multicolumn{1}{l}{68.36} & \multicolumn{1}{l}{\underline{68.89}} & \multicolumn{1}{l}{\textbf{68.95}}\\

    & & \multicolumn{1}{l}{mAP} & \multicolumn{1}{l}{78.68} & \multicolumn{1}{l}{79.06} & \multicolumn{1}{l}{78.52} & \multicolumn{1}{l}{78.62} & \multicolumn{1}{l}{\underline{79.43}} & \multicolumn{1}{l}{\textbf{79.66}}\\

    & & \multicolumn{1}{l}{mIoU} & \multicolumn{1}{l}{49.29} & \multicolumn{1}{l}{49.68} & \multicolumn{1}{l}{49.03} & \multicolumn{1}{l}{49.11} & \multicolumn{1}{l}{\underline{49.91}} & \multicolumn{1}{l}{\textbf{50.24}}\\
    
    & & \multicolumn{1}{l}{mF1} & \multicolumn{1}{l}{32.92} & \multicolumn{1}{l}{33.83} & \multicolumn{1}{l}{32.28} & \multicolumn{1}{l}{32.56} & \multicolumn{1}{l}{\underline{34.11}} & \multicolumn{1}{l}{\textbf{34.26}}\\
    \bottomrule
  \end{tabular}}

  \end{center}
  \vspace{-2mm}

\end{table}
